Universal approximation property of invertible neural networks

Invertible neural networks (INNs) are neural network architectures with invertibility by design. Thanks to their invertibility and the tractability of Jacobian, INNs have various machine learning applications such as probabilistic modeling, generative modeling, and representation learning. However, their attractive properties often come at the cost of restricting the layer designs, which poses a question on their representation power: can we use these models to approximate sufficiently diverse functions? To answer this question, we have developed a general theoretical framework to investigate the representation power of INNs, building on a structure theorem of differential geometry. The framework simplifies the approximation problem of diffeomorphisms, which enables us to show the universal approximation properties of INNs. We apply the framework to two representative classes of INNs, namely Coupling-Flow-based INNs (CF-INNs) and Neural Ordinary Differential Equations (NODEs), and elucidate their high representation power despite the restrictions on their architectures.

==> 0_author_footnotes.tex <==
\def\thefootnote{\(\dagger\)}\footnotetext{These authors contributed equally to this work.}\def\thefootnote{\arabic{footnote}}

==> 0_metadata.tex <==

\newcommand{\shortTitle}{Universality of Invertible Neural Networks}
\newcommand{\titleText}{Universal Approximation Property of \\ Invertible Neural Networks}
\newcommand{\titleSentenceCase}{Universal approximation property of invertible neural networks}
\ShortHeadings{\shortTitle{}}{Ishikawa, Teshima, Tojo, Oono, Ikeda, and Sugiyama}
\firstpageno{1}
\title{\titleText{}}

\author{\name Isao Ishikawa\textsuperscript{\(\dagger\)} \email ishikawa.isao.zx@ehime-u.ac.jp\\
      \addr Ehime University, RIKEN\\
      Ehime, JAPAN
    \AND
      \name Takeshi Teshima\textsuperscript{\(\dagger\)}\thanks{This work was done when the author was with The University of Tokyo and RIKEN.} \email takeshi.teshima@a.riken.jp \\
       \addr The University of Tokyo, RIKEN\\
       Tokyo, JAPAN
    \AND
      \name Koichi Tojo \email koichi.tojo@riken.jp\\
      \addr Center for Advanced Intelligence Project\\
      RIKEN\\
      Tokyo, JAPAN
    \AND
      \name Kenta Oono \email kenta.oono@a.riken.jp\\
      \addr Center for Advanced Intelligence Project\\
      RIKEN\\
      Tokyo, JAPAN
    \AND
      \name Masahiro Ikeda \email masahiro.ikeda@riken.jp\\
      \addr Center for Advanced Intelligence Project\\
      RIKEN\\
      Tokyo, JAPAN
    \AND
      \name Masashi Sugiyama \email sugi@k.u-tokyo.ac.jp\\
      \addr Center for Advanced Intelligence Project\\
      RIKEN, The University of Tokyo\\
      Tokyo, JAPAN
}

\editor{}


\hypersetup{
pdftitle={},
pdfsubject={},
pdfauthor={},
pdfkeywords={Invertible neural network, Normalizing flow, Affine coupling, Neural ordinary differential equations, Diffeomorphism, Universal approximation property, Universality},
}


==> A_C_IPM_backup_1.tex <==
\subsection{General Integral Probability Metric}\label{appendix: IPM}

The results in Subsection~\ref{sec:proof-of-generalized-distributional-universality} implies the universality of INNs with respect to the total variation (TV) topology.
Here, we consider how the theoretical guarantees in the TV topology can be transported to other notions of closeness, namely those of integral probability metrics (IPMs).

IPMs are defined as follows.
\begin{definition}[Integral probability metric; \citet{MullerIntegral1997}]
Let \(\vIPMBaseSp\) be a measurable space, \(\mu\) and \(\nu\) be probability measures on \(\vIPMBaseSp\), and \(\vIPMClass\) be \(\Re\)-valued bounded measurable functions on \(\vIPMBaseSp\).
Then, the \emph{integral probability metric} (IPM) based on \(\vIPMClass\) is defined as
\[
\IPM{\vIPMClass}{\mu, \nu} := \sup_{\vIPMFn \in \vIPMClass} \left| \int_\vIPMBaseSp \vIPMFn d\mu - \int_\vIPMBaseSp \vIPMFn d\nu \right|
\]
\end{definition}
For a comprehensive review on IPMs, see, e.g., \citet{SriperumbudurIntegral2009}.

By selecting appropriate \(\vIPMClass\), various distance measures in probability theory and statistics can be obtained as special cases of the IPM.
In the following, assume that \(\vIPMBaseSp\) is equipped with a distance metric \(\vIPMBaseDist\) and that the \(\sigma\)-algebra is the Borel \(\sigma\)-algebra induced by the metric topology of \(\vIPMBaseDist\).
Let \(\Lipnorm{f} := \sup_{x, y \in \vIPMBaseSp, x \neq y} \frac{|f(x) - f(y)|}{\vIPMBaseDist(x, y)}\) and \(\bddLipnorm{f} := \inftynorm{f} + \Lipnorm{f}\).
Let \(\vRKHS\) be a reproducing kernel Hilbert space (RKHS) induced by a reproducing kernel \(\vRKHSkern: \vIPMBaseSp \times \vIPMBaseSp \to \Re\), and let \(\RKHSnorm{\cdot}\) be its RKHS norm.
\begin{definition}[\citet{SriperumbudurIntegral2009}]
We define the following metrics.
\begin{itemize}
    \item \emph{Dudley Metric}: \(\cIPMDudley = \{f: \bddLipnorm{f} \leq 1\}\) yields the Dudley metric \(\IPM{\cIPMDudley}{\mu, \nu}\).
    \item \emph{Wasserstein distance}: if \(\vIPMBaseSp\) is separable, then \(\cIPMOneWasserstein = \{f: \Lipnorm{f} \leq 1\}\) yields the \(1\)-Wasserstein distance \(\IPM{\cIPMOneWasserstein}{\mu, \nu}\) for \(\mu, \nu \in \cOneWassersteinDists = \{\nu': \int \vIPMBaseDist(x, y) d\nu'(x)<\infty, \forall y \in \vIPMBaseSp\}\).
    \item \emph{Total variation distance}: \(\cIPMTV = \{f: \inftynorm{f} \leq 1\}\) yields the total variation distance \(\IPM{\cIPMTV}{\mu, \nu}\).
    \item \emph{Maximum mean discrepancy} (MMD): selecting \(\vIPMClass = \cIPMMMD = \{f \in \vRKHS: \RKHSnorm{f} \leq 1\}\) yields the MMD \(\IPM{\cIPMMMD}{\mu, \nu}\).
\end{itemize}
\end{definition}

We have the following relations that immediately follow from the definitions.
\begin{proposition}
We have \(\IPM{\cIPMDudley}{\mu, \nu} \leq \IPM{\cIPMTV}{\mu, \nu}\).

\end{proposition}
\begin{proof}
The first inequality is immediate from the definition since \(\cIPMDudley \subset \cIPMTV\).
\end{proof}

The following is a well-known inequality for the relation between the Wasserstein distance and the total variation distance.
\begin{fact}[{\citealp{VillaniOptimal2009}, Theorem~6.15}]\label{fact: Wasserstein bound bdd by TV}
Let \((\vIPMBaseSp, \vIPMBaseDist)\) be a separable complete metric space, and \(\mu\) and \(\nu\) be probability measures on \(\vIPMBaseSp\).
Suppose \(\vIPMBaseSp\) is bounded with diameter \(R\).
Then, we have \(\IPM{\cIPMOneWasserstein}{\mu, \nu} \leq R \cdot \IPM{\cIPMTV}{\mu, \nu}\).
\end{fact}

The following is an immediate corollary of this fact.
It has an interpretation that the distributional universality with respect to the TV topology implies a representation power guarantee with respect to the Wasserstein distance for probability distributions with bounded support.
\begin{corollary}\label{cor: TV to bdd Wasserstein}
Suppose $\mathcal{M}$ is a $(\mathcal{P}^{\rm TV}, \mu)$-distributional universal approximator for $\mathcal{P}_{\rm ab}$ with $\mu \in \mathcal{P}_{\rm ab}$.
Let \(\nu \in \mathcal{P}_{\rm ab}\), assume \(\nu\) has bounded support, and \(K \subset \ReD\) be any bounded measurable subset such that \(\supp{\nu} \subset K\).
Then, for any \(\varepsilon > 0\), there exists \(g \in \mathcal{M}\) such that \(\IPM{\cIPMOneWasserstein}{\truncate{K}{\pushforward{g}{\mu}},\nu} < \varepsilon\), where \(\truncate{K}{\eta} := \eta(\cdot \cap K) / \eta(K)\) for a probability distribution \(\eta\) with \(\eta(K) > 0\).
\end{corollary}
\begin{proof}
Since \((K, \|\cdot\|)\) is a separable complete metric space, we have, by applying Fact~\ref{fact: Wasserstein bound bdd by TV} with \(\truncate{K}{\pushforward{g}{\mu}}\) and \(\nu\),
\begin{align*}
\IPM{\cIPMOneWasserstein}{\truncate{K}{\pushforward{g}{\mu}},\nu}
&= \sup_{f \in \cIPMOneWasserstein} \left|\int_{\ReD} f d(\truncate{K}{\pushforward{g}{\mu}}) - \int_{\ReD} f d\nu\right| \\
&= \sup_{f \in \Restrict{\cIPMOneWasserstein}{K}} \left|\int_K f d(\truncate{K}{\pushforward{g}{\mu}}) - \int_K f d\nu\right| \\
&\leq \diam{K}\sup_{A'} |\truncate{K}{\pushforward{g}{\mu}}(A') - \nu(A')| =: \text{(RHS)},
\end{align*}
where \(\sup_{A'}\) denotes the supremum over all measurable subsets of \(K\), and \(\Restrict{\cIPMOneWasserstein}{K} := \{\Restrict{f}{K}: f \in \cIPMOneWasserstein\}\).
The right-hand side (RHS) is further bounded as
\begin{align*}
\text{(RHS)}
&= \diam{K}\sup_{A} |\pushforward{g}{\mu}(A \cap K)/\pushforward{g}{\mu}(K) - \nu(A \cap K)| \\
&\leq \diam{K}\sup_{A} |\pushforward{g}{\mu}(A)/\pushforward{g}{\mu}(K) - \nu(A)|,
\end{align*}
where \(\sup_{A}\) denotes the supremum over all measurable subsets of \(\ReD\), and the inequality holds since \(\sup_{A}\) runs through all the measurable subsets of the form \(A \cap K\) as well.
Now,
\begin{align*}
\left|\frac{\pushforward{g}{\mu}(A)}{\pushforward{g}{\mu}(K)} - \nu(A)\right|
&\leq \frac{|\pushforward{g}{\mu}(A) - \nu(A)|}{\pushforward{g}{\mu}(K)} + \left|\frac{1}{\pushforward{g}{\mu}(K)} - 1\right| \nu(A) \\
&= \frac{|\pushforward{g}{\mu}(A) - \nu(A)|}{\pushforward{g}{\mu}(K)} + \left|\nu(K) - \pushforward{g}{\mu}(K)\right| \frac{\nu(A)}{\pushforward{g}{\mu}(K)} \\
&\leq \frac{1 + \nu(A)}{\pushforward{g}{\mu}(K)}\IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu}.
\end{align*}
Since we have \(\nu(K) - \pushforward{g}{\mu}(K) \leq |\pushforward{g}{\mu}(K) - \nu(K)| \leq \IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu}\) by the triangle inequality, we further obtain \(1 - \IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu} \leq \pushforward{g}{\mu}(K)\).
Therefore, for any \(g \in \mathcal{M}\) such that \(\IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu} < 1\),
we have
\[
\IPM{\cIPMOneWasserstein}{\truncate{K}{\pushforward{g}{\mu}},\nu}
\leq \diam{K} \frac{2 \cdot \IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu}}{1 - \IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu}}.
\]
Thus, by the hypothesis on the $(\mathcal{P}^{\rm TV}, \mu)$-distributional universal approximation property, we have the assertion.
\end{proof}

==> A_C_IPM_backup_2.tex <==
\subsection{Integral Probability Metrics}\label{appendix: IPM}

The results in Subsection~\ref{sec:proof-of-generalized-distributional-universality} implies the universality of INNs with respect to the total variation (TV) topology.
Here, we consider how the theoretical guarantees in the TV topology can be transported to other notions of closeness, namely those of integral probability metrics (IPMs).

We say a measurable set $A \subset \R^n$ is a {\em continuity set} of a measure \(\mu\) if the boundary $\partial A$ of $A$ is a null set, i.e., \(\mu(\partial A) = 0\).
We say a measurable set $A \subset \Re^n$ is a \emph{non-null set} of a measure \(\mu\) if \(\mu(A) \neq 0\).
For any measurable subset \(K \subset \Re^n\) and any probability measure \(\eta\) on \(\Re^n\), let us define the truncated measure \(\truncate{K}{\eta} := \eta(\cdot \cap K) / \eta(K)\) if \(\eta(K) > 0\) and \(\truncate{K}{\eta} := \zeroMeasure\) if \(\eta(K) = 0\), where \(\zeroMeasure\) is a constant zero measure.
To state the results, we define the following notion of universality.

\begin{definition}[Compact distributional universality]\label{def: compact distributional universality}
Let $\INNModelGeneric$ be a model which is a set of measurable maps from $\R^m$ to $\R^n$.
Let $\mathcal{P}_0$ be a set of probability measures on $\R^n$ with some topology. % that is closed under truncation by the open bounded sets of $\R^n$.
Let $\mathcal{Q}$ be a subset of \(\mathcal{P}_0\).
Fix a probability measure $\mu_0$ on $\Re^m$.
We say that a model $\INNModelGeneric$ is a \emph{$(\mathcal{P}_0, \mu_0)$-compact-distributional universal approximator} for $\mathcal{Q}$ (or \emph{has the $(\mathcal{P}_0, \mu_0)$-compact-distributional universal approximation property} for $\mathcal{Q}$) if for any \(\nu \in \mathcal{Q}\) and any non-null compact continuity set \(K \subset \Re^n\) of \(\nu\), $\{\truncate{K}{(g_*\mu_0)}: g \in \INNModelGeneric\} \setminus \{\zeroMeasure\}$ is a subset of $\mathcal{P}_0$ and if its closure (in $\mathcal{P}_0$) contains $\truncate{K}{\nu}$.
\end{definition}
Note, in particular, that if \(\nu\) is compactly supported and \(K\) is such that \(\supp{\nu} \subset \interior{K}\), where \(\interior{K}\) denotes the interior of \(K\), then \(K\) is a continuity set of \(\nu\). Also, in this case, \(\truncate{K}{\nu} = \nu\).
Therefore the compact distributional universality includes, as special cases, the assertions that \(\nu\) can be approximated by \(\{\truncate{K}{(\pushforward{g}{\mu_0})}\}_{g \in \mathcal{M}}\) in terms of the topology of \(\mathcal{P}_0\) for any sufficiently large compact set \(K\).
\begin{remark}
Let us consider connection between the compact distributional universality and the usual distributional universality (Definition \ref{def: dist. univ. approx.}).
Let $\mathcal{P}_0$ be a set of probability measures on $\R^n$ with some topology.
For $\mu \in \mathcal{P}_0$, a compact continuity set $K$ of $\mu$, and a neighborhood $V$ of $\mu|_K$ with $\mu|_K \neq \zeroMeasure$, we define
\[W_V(\mu;K) := \{ \nu \in \mathcal{P}_0 : \nu|_K \in V \}.  \]
We define a new topology of $\mathcal{P}_0$ via the neighborhoods of $\mu$'s by those generated by $W_V(\mu;K)$'s.
We denote by $\mathcal{P}_0^\tau$ the set $\mathcal{P}_0$ equipped with the above new topology.
By definition, the truncation $\cdot|_K: \mathcal{P}_0^\tau \to \mathcal{P}_0 \cup \{\zeroMeasure\}$ for any compact continuity set of $\mu$ is continuous at arbitrary $\mu$ with $\mu|_K \neq \zeroMeasure$ is continuous, where the topology of $\mathcal{P}_0 \cup \{\zeroMeasure\}$ is the direct sum topology.
Conversely, $\mathcal{P}_0^\tau$ is characterized as the set $\mathcal{P}_0$ equipped with the weakest topology such that the above truncations are continuous.
\end{remark}


IPMs are defined as follows.
\begin{definition}[Integral probability metric; \citet{MullerIntegral1997}]
Let \(\vIPMBaseSp\) be a measurable space, \(\mu\) and \(\nu\) be probability measures on \(\vIPMBaseSp\), and \(\vIPMClass\) be \(\Re\)-valued bounded measurable functions on \(\vIPMBaseSp\).
Then, the \emph{integral probability metric} (IPM) based on \(\vIPMClass\) is defined as
\[
\IPM{\vIPMClass}{\mu, \nu} := \sup_{\vIPMFn \in \vIPMClass} \left| \int_\vIPMBaseSp \vIPMFn d\mu - \int_\vIPMBaseSp \vIPMFn d\nu \right|
\]
\end{definition}
For a comprehensive review on IPMs, see, e.g., \citet{SriperumbudurIntegral2009}.

By selecting appropriate \(\vIPMClass\), various distance measures in probability theory and statistics can be obtained as special cases of the IPM.
In the following, assume that \(\vIPMBaseSp\) is equipped with a distance metric \(\vIPMBaseDist\) and that the \(\sigma\)-algebra is the Borel \(\sigma\)-algebra induced by the metric topology of \(\vIPMBaseDist\).
Let \(\Lipnorm{f} := \sup_{x, y \in \vIPMBaseSp, x \neq y} \frac{|f(x) - f(y)|}{\vIPMBaseDist(x, y)}\) and \(\bddLipnorm{f} := \inftynorm{f} + \Lipnorm{f}\).
Let \(\vRKHS\) be a reproducing kernel Hilbert space (RKHS) induced by a positive semidefinite kernel \(\vRKHSkern: \vIPMBaseSp \times \vIPMBaseSp \to \Re\), and let \(\RKHSnorm{\cdot}\) be its RKHS norm.
\begin{definition}[\citet{SriperumbudurIntegral2009}]
We define the following metrics.
\begin{itemize}
    \item \emph{Dudley Metric}: \(\cIPMDudley = \{f: \bddLipnorm{f} \leq 1\}\) yields the Dudley metric \(\IPM{\cIPMDudley}{\mu, \nu}\).
    \item \emph{Wasserstein distance}: if \(\vIPMBaseSp\) is separable, then \(\cIPMOneWasserstein = \{f: \Lipnorm{f} \leq 1\}\) yields the \(1\)-Wasserstein distance \(\IPM{\cIPMOneWasserstein}{\mu, \nu}\) for \(\mu, \nu \in \cOneWassersteinDists = \{\nu': \int \vIPMBaseDist(x, y) d\nu'(x)<\infty, \forall y \in \vIPMBaseSp\}\).
    \item \emph{Total variation distance}: \(\cIPMTV = \{f: \inftynorm{f} \leq 1\}\) yields the total variation distance \(\IPM{\cIPMTV}{\mu, \nu}\).
    \item \emph{Maximum mean discrepancy} (MMD): selecting \(\cIPMMMD = \{f \in \vRKHS: \RKHSnorm{f} \leq 1\}\) yields the MMD \(\IPM{\cIPMMMD}{\mu, \nu}\).
\end{itemize}
We use \(\mathcal{P}^{\cTextDudley}\), \(\mathcal{P}^{\cTextOneWasserstein}\), and \(\mathcal{P}^{\cTextMMD}\), to denote \(\mathcal{P}\) equipped with the induced topology of \(\IPM{\cIPMDudley}{\cdot,\cdot}\), \(\IPM{\cIPMOneWasserstein}{\cdot,\cdot}\), and \(\IPM{\cIPMMMD}{\cdot,\cdot}\), respectively.
\end{definition}

We have the following elementary relations that can be easily shown from the definitions.
\begin{proposition}\label{prop: TV-Dudley-MMD}
We have the following inequalities:
\begin{align*}
\IPM{\cIPMDudley}{\mu, \nu} &\leq \IPM{\cIPMTV}{\mu, \nu}, \\
\IPM{\cIPMMMD}{\mu, \nu} &\leq
\left(\sup_{x \in \vIPMBaseSp} \vRKHSkern(x, x)\right)^{\frac{1}{2}} \IPM{\cIPMTV}{\mu, \nu}.
\end{align*}
\end{proposition}
\begin{proof}
The first inequality follows from \(\cIPMDudley \subset \cIPMTV\), which holds by definition.
The second inequality follows from the Cauchy-Schwarz inequality:
\[
\inftynorm{f} = \sup_{x \in \vIPMBaseSp} |f(x)|
= \sup_{x \in \vIPMBaseSp} |\langle f, \vRKHSkern(x, \cdot) \rangle_{\vRKHS}|
\leq \RKHSnorm{f} \left(\sup_{x \in \vIPMBaseSp} \vRKHSkern(x, x)\right)^{\frac{1}{2}},
\]
where \(\langle \cdot, \cdot \rangle_{\vRKHS}\) denotes the inner product of \(\vRKHS\).
\end{proof}

We also have the following relation between the total variation distance and the \(1\)-Wasserstein distance for \(\vIPMBaseSp = \ReD\).
\begin{lemma}\label{lem: TV-W1}
Suppose $\mathcal{M}$ is a $(\mathcal{P}^{\rm TV}, \mu)$-distributional universal approximator for $\mathcal{Q} \subset \mathcal{P}^{\rm TV}$ with $\mu \in \mathcal{P}^{\rm TV}$.
Let \(\nu \in \mathcal{Q}\), and let \(K \subset \ReD\) be any compact subset.
Then, for any \(\varepsilon > 0\), there exists \(g \in \mathcal{M}\) such that \(\IPM{\cIPMOneWasserstein}{\truncate{K}{\pushforward{g}{\mu}},\nu} < \varepsilon\).
\end{lemma}
We defer the proof of Lemma~\ref{lem: TV-W1} to the bottom part of this subsection, and we first display the following proposition to collect Corollary~\ref{prop: TV-Dudley-MMD} and Lemma~\ref{lem: TV-W1}.
\begin{proposition}\label{prop: TV-univ to Dudley, MMD, and W1}
Let \(\mathcal{Q} \subset \mathcal{P}\) and $\mu \in \mathcal{P}$.
Assume that $\mathcal{M}$ is a $(\mathcal{P}^{\rm TV}, \mu)$-distributional universal approximator for $\mathcal{Q}$.
Then, we have the following.
\begin{itemize}
    \item[(a)] $\mathcal{M}$ is a $(\mathcal{P}^{\cTextDudley}, \mu)$-distributional universal approximator for $\mathcal{Q}$,
    \item[(b)] If \(\sup_{x \in \ReD} \vRKHSkern(x, x) < \infty\), then $\mathcal{M}$ is a $(\mathcal{P}^{\cTextMMD}, \mu)$-distributional universal approximator for $\mathcal{Q}$,
    \item[(c)] $\mathcal{M}$ is a $(\mathcal{P}^{\cTextOneWasserstein}, \mu)$-compact-distributional universal approximator for $\mathcal{Q}$.
\end{itemize}
\end{proposition}
The condition part of Proposition~\ref{prop: TV-univ to Dudley, MMD, and W1} is covered by the conclusion part of Theorem~\ref{thm: univ aprox for 0inf11 induces distribution TV approximator}, where \(\mathcal{Q}\) and \(\mu\) are arbitrary \(\mathcal{Q} \subset \mathcal{P}_{\rm ab}\) and \(\mu \in \mathcal{P}_{\rm ab}\).
Therefore, we can immediately obtain the theoretical guarantee of distribution approximation using INNs with respect to these IPMs given a Sobolev universality of \(\mathcal{M}\).
\begin{proof}[Proof of Proposition~\ref{prop: TV-univ to Dudley, MMD, and W1}]
The first two immediately follow from Corollary~\ref{prop: TV-Dudley-MMD}, and the last assertion follows from Lemma~\ref{lem: TV-W1}.
\end{proof}

To prove Lemma~\ref{lem: TV-W1}, we use the following well-known inequality between the Wasserstein distance and the total variation distance.
\begin{fact}[{\citealp{VillaniOptimal2009}, Theorem~6.15}]\label{fact: Wasserstein bound bdd by TV}
Let \((\vIPMBaseSp, \vIPMBaseDist)\) be a separable complete metric space that is bounded with diameter \(R\), and \(\mu\) and \(\nu\) be probability measures on \(\vIPMBaseSp\).
Then, we have \(\IPM{\cIPMOneWasserstein}{\mu, \nu} \leq R \cdot \IPM{\cIPMTV}{\mu, \nu}\).
\end{fact}

Lemma~\ref{lem: TV-W1} is an immediate corollary of this fact.
\begin{proof}[Proof of Lemma~\ref{lem: TV-W1}]
Since \((K, \|\cdot\|)\) is a separable complete metric space, we have, by applying Fact~\ref{fact: Wasserstein bound bdd by TV} with \(\truncate{K}{\pushforward{g}{\mu}}\) and \(\nu\),
\begin{align*}
\IPM{\cIPMOneWasserstein}{\truncate{K}{\pushforward{g}{\mu}},\nu}
&= \sup_{f \in \cIPMOneWasserstein} \left|\int_{\ReD} f d(\truncate{K}{\pushforward{g}{\mu}}) - \int_{\ReD} f d\nu\right| \\
&= \sup_{f \in \Restrict{\cIPMOneWasserstein}{K}} \left|\int_K f d(\truncate{K}{\pushforward{g}{\mu}}) - \int_K f d\nu\right| \\
&\leq \diam{K}\sup_{A'} |\truncate{K}{\pushforward{g}{\mu}}(A') - \nu(A')| =: \text{(RHS)},
\end{align*}
where \(\sup_{A'}\) denotes the supremum over all measurable subsets of \(K\), and \(\Restrict{\cIPMOneWasserstein}{K} := \{\Restrict{f}{K}: f \in \cIPMOneWasserstein\}\).
The right-hand side (RHS) is further bounded as
\begin{align*}
\text{(RHS)}
&= \diam{K}\sup_{A} |\pushforward{g}{\mu}(A \cap K)/\pushforward{g}{\mu}(K) - \nu(A \cap K)| \\
&\leq \diam{K}\sup_{A} |\pushforward{g}{\mu}(A)/\pushforward{g}{\mu}(K) - \nu(A)|,
\end{align*}
where \(\sup_{A}\) denotes the supremum over all measurable subsets of \(\ReD\), and the inequality holds since \(\sup_{A}\) runs through all the measurable subsets of the form \(A \cap K\) as well.
Now,
\begin{align*}
\left|\frac{\pushforward{g}{\mu}(A)}{\pushforward{g}{\mu}(K)} - \nu(A)\right|
&\leq \frac{|\pushforward{g}{\mu}(A) - \nu(A)|}{\pushforward{g}{\mu}(K)} + \left|\frac{1}{\pushforward{g}{\mu}(K)} - 1\right| \nu(A) \\
&= \frac{|\pushforward{g}{\mu}(A) - \nu(A)|}{\pushforward{g}{\mu}(K)} + \left|\nu(K) - \pushforward{g}{\mu}(K)\right| \frac{\nu(A)}{\pushforward{g}{\mu}(K)} \\
&\leq \frac{1 + \nu(A)}{\pushforward{g}{\mu}(K)}\IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu}.
\end{align*}
Since we have \(\nu(K) - \pushforward{g}{\mu}(K) \leq |\pushforward{g}{\mu}(K) - \nu(K)| \leq \IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu}\) by the triangle inequality, we further obtain \(1 - \IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu} \leq \pushforward{g}{\mu}(K)\).
Therefore, for any \(g \in \mathcal{M}\) such that \(\IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu} < 1\),
we have
\[
\IPM{\cIPMOneWasserstein}{\truncate{K}{\pushforward{g}{\mu}},\nu}
\leq \diam{K} \frac{2 \cdot \IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu}}{1 - \IPM{\cIPMTV}{\pushforward{g}{\mu}, \nu}}.
\]
Thus, by the hypothesis on the $(\mathcal{P}^{\rm TV}, \mu)$-distributional universal approximation property, we have the assertion.
\end{proof}
